Box2Mask: Weakly Supervised 3D Semantic Instance Segmentation Using Bounding Boxes

Current 3D segmentation methods heavily rely on large-scale point-cloud datasets, which are notoriously laborious to annotate. Few attempts have been made to circumvent the need for dense per-point annotations. In this work, we look at weakly-supervised 3D semantic instance segmentation. The key idea is to leverage 3D bounding box labels which are easier and faster to annotate. Indeed, we show that it is possible to train dense segmentation models using only bounding box labels. At the core of our method, \name{}, lies a deep model, inspired by classical Hough voting, that directly votes for bounding box parameters, and a clustering method specifically tailored to bounding box votes. This goes beyond commonly used center votes, which would not fully exploit the bounding box annotations. On ScanNet test, our weakly supervised model attains leading performance among other weakly supervised approaches (+18 mAP@50). Remarkably, it also achieves 97% of the mAP@50 score of current fully supervised models. To further illustrate the practicality of our work, we train Box2Mask on the recently released ARKitScenes dataset which is annotated with 3D bounding boxes only, and show, for the first time, compelling 3D instance segmentation masks.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

==> tables/scannet_val_instance.tex <==
% !TEX root = ../main.tex
\begin{table}
\setlength{\tabcolsep}{5px}%
\begin{center}
    \begin{tabular}{l c c c c c c c}
        \toprule
        \multicolumn{8}{c}{{3D Semantic Instance Segmentation Scores on ScanNet}}  \\ 
            \midrule
            \multirow{2}{*}{\hspace{3mm} }  & \multicolumn{3}{c}{Validation Set} & & \multicolumn{3}{c}{Hidden Test Set}\\
           \cmidrule(r){2-4} \cmidrule(r){6-8}
          & mAP & \small{@50\%} & \small{@25\%} & \hspace{3px} & mAP & \small{@50\%} & \small{@25\%}\\
        \midrule

         \hline
          \textbf{Weak Supervision Models}                              & \multicolumn{3}{c}{  } & &   &   & \\
        \midrule
         CSC~\cite{Hou21CVPR} (20 Pts + Centers)        & -     &  26.3    &     -      & & 15.9    & 28.9    & 49.6 \\
         PC~\cite{Xie20ECCV} (20 Pts + Centers) & -     & -     &     -      & & 12.4    & 25.9    & 47.4 \\
         CSC~\cite{Hou21CVPR} (50 Pts + Centers)        & -     & 32.6     &     -      & & 22.9    &   41.4  & 62.0 \\
         PC~\cite{Xie20ECCV} (50 Pts + Centers)  & -     & -     &    -       & & 21.6    & 40.0    & 60.3 \\
         CSC~\cite{Hou21CVPR} (100 Pts + Centers)        & -     & 39.9     &    -       & & 25.8    & 46.0    & 65.4 \\
         PC~\cite{Xie20ECCV} (100 Pts + Centers) & -     & -     &    -       & & 25.6    & 45.6    & 63.7 \\
         CSC~\cite{Hou21CVPR} (200 Pts + Centers)        & -     & 48.9     &    -       & & 29.3    & 49.4    & 70.2 \\
         PC~\cite{Xie20ECCV} (200 Pts + Centers) & -     & 44.5     &    -       & & 27.8    & 47.1    & 66.2 \\
        %\hline
        
         \textbf{Ours} (BBs, X Centers + Size)     & \textbf{39.1} &  \textbf{59.7} &    \textbf{71.8}          & & -    & -    & - \\

        \midrule
          \textbf{Full Supervision Models}               & \multicolumn{3}{c}{ } & &   &   & \\
        \midrule
          3D-SIS~\cite{Hou19CVPR}   	& -     & 18.7  & 35.7 		& & 16.1 & 38.2 & 55.8\\
          3D-BoNet~\cite{Yang19NIPS} 	& -  	& -  	& - 		& & 25.3 & 48.8 & 68.7\\
          MTML~\cite{Lahoud19ICCV}  	& 20.3  & 40.2  & 55.4 		& & 28.2 & 54.9 & 73.1\\
          3D-MPA~\cite{Engelmann20CVPR} & 35.3  & 59.1  & 72.4      & & 35.5 & 61.1 & 73.7\\
          HAIS~\cite{Chen21ICCV}        & 43.5  & 64.1  & \textbf{75.6}      & & 45.7 & 69.9 & 80.3\\
          SSTNet~\cite{Liang21CVPR}     & \textbf{49.4}  & 64.3  & 74.0      & & 50.6 & 69.8 & 78.9\\

         \bottomrule
    \end{tabular}
\end{center}
\caption{
\textbf{3D instance segmentation scores ScanNetV2}~\cite{Dai17CVPR}. The metric is mean average precision (mAP) at an IoU threshold of 25\%, 50\% and averaged over the range [0.5:0.95:05]. IoU on per-point instance masks. \julian{Keep Centers + Size notation, or switch back to "BB Supervision"?}}
\label{tab:inst_scannet}
\end{table}


==> tables/stanford_a5_instance.tex <==
% !TEX root = ../main.tex
\begin{table}
\setlength{\tabcolsep}{5px}%
\begin{center}

    \begin{tabular}{l c c c c c c c}
        \toprule
        \multicolumn{6}{c}{3D Semantic Instance Segmentation Scores on S3DIS}  \\ 
            \midrule
            \multirow{2}{*}{\hspace{3mm} }  & \multicolumn{2}{c}{Area 5} & & \multicolumn{2}{c}{6-fold CV}\\
           \cmidrule(r){2-3} \cmidrule(r){5-6}
          & mPrec & mRec  & \hspace{3px} & mPrec & mRec \\
          \midrule
          \midrule
              \textbf{Full Supervision}  &      &                & &     &      \\
        \midrule
          ASIS\,\cite{Wang19CVPR}           & 55.3     & 42.4                & & 63.6    & 47.5     \\
          3D-BoNet\,\cite{Yang19NIPS} 	    & -     & -                & & 65.6    & 47.6     \\
          3D-MPA\,\cite{Engelmann20CVPR}     & 46.7     & \textbf{65.6}                & & 66.7    & 64.1    \\
          PointGroup\,\cite{Jiang20CVPR}  	& 61.9     & 62.1                & & 69.6    & 69.2    \\
          OccuSeg\,\cite{Han20CVPR}  	    & -     & -                & & 72.8    & 60.3     \\
          HAIS\,\cite{Chen21ICCV}            & \textbf{71.1}     & 65.0                & & 73.2    & 69.4    \\
          SSTNet\,\cite{Liang21CVPR}        & 65.5     & 64.2                & & 73.5    & \textbf{73.4}    \\

    \midrule
    \textbf{Weak Supervision}  &      &                & &     &      \\
         \midrule
         {{\name{} (ours) (BB supervision)}}        &{66.7}     & {65.5}                & & {72.2}    & {70.5}    \\
         \bottomrule
    \end{tabular}
\end{center}
\caption{
\textbf{3D instance segmentation scores on S3DIS\,\cite{Armeni16CVPR}}}
\label{tab:instance_scores_stanford}
\end{table}

